Prompting-based Temporal Domain Generalization

Machine learning traditionally assumes that the training and testing data are distributed independently and identically. However, in many real-world settings, the data distribution can shift over time, leading to poor generalization of trained models in future time periods. This paper presents a novel prompting-based approach to temporal domain generalization that is parameter-efficient, time-efficient, and does not require access to future data during training. Our method adapts a trained model to temporal drift by learning global prompts, domain-specific prompts, and drift-aware prompts that capture underlying temporal dynamics. Experiments on classification, regression, and time series forecasting tasks demonstrate the generality of the proposed approach. The code repository will be publicly shared.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> paper_planning.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\caption{Paper Planning: Feel free to change orders of steps.}
\begin{tabular}{ll|l|l|l}
\rowcolor[HTML]{EFEFEF} 
\textbf{Section} & \textbf{Notes} &\textbf{First Draft ready?} & \textbf{Review-ready?} & \textbf{Final-ready?} \\

\rowcolor[HTML]{FFCCC9} \textbf{Title}                 & Iterate later&  Done &   &    \\

\rowcolor[HTML]{FFCE93} \textbf{Paper skeleton}        & Section headings. &  Done & &     \\

\rowcolor[HTML]{FFFFC7} \textbf{Intro skeleton}        & A bullet list of points to make. & Done  & &     \\
\rowcolor[HTML]{FFFFC7} \textbf{Intro body}            & NA& Done  & &   \\

\rowcolor[HTML]{9AFF99} \textbf{Related work skeleton} & List of related topics/papers& Done  &  &      \\
\rowcolor[HTML]{9AFF99} \textbf{Related work body}     & NA & Done  &  &     \\
\rowcolor[HTML]{96FFFB} \textbf{Approach skeleton}     & NA  & Done  &  &   \\
\rowcolor[HTML]{96FFFB} \textbf{Approach figures}         &NA &  Done    &   & \\
\rowcolor[HTML]{96FFFB} \textbf{Approach body}         &NA &   8/23 &   & \\

\rowcolor[HTML]{ECF4FF} \textbf{Results skeleton}      &NA & Done   &     &\\
\rowcolor[HTML]{ECF4FF} \textbf{Results body}          & NA & 8/24 &   &     \\

\rowcolor[HTML]{CBCEFB} \textbf{Conclusion/abstract}   &NA&   &  &     \\

\rowcolor[HTML]{FFCE93} \textbf{Supple. material}      &NA&    & &     \\

\end{tabular}
\end{table*}



==> sections/algorithm.tex <==

\begin{algorithm*}
\caption{Training Procedure }
\begin{algorithmic}[1]
\Require
    Source domains $\{D_t | 1 \leq t \leq \tau\}$,
    Target domains $\{D_t | t > \tau\}$,
    Pre-trained model to adapt $f_\theta$ parameterized by $\theta$,
    Temporal prompt generator $g_\omega$ parameterized by $\omega$,
    Labeled data from source domains $D_1, D_2, \ldots, D_\tau$
\Ensure
    Domain-specific prompts $P_{S1}, P_{S2}, \ldots, P_{S\tau}$,
    Temporal prompts $P_{T2}, P_{T3}, \ldots, P_{T\tau+1}$
    Generic prompt $P_G$

\Procedure{DomainSpecificPromptLearning}{}
    \For{each domain $D_t$ in $\{D_t | 1 \leq t \leq \tau\}$}
        \State Prepend  $X$ with $P_{S(t)}$
        \State Process combined input $[P_{S(t)}; X]$ using frozen backbone $f_\theta$
        \State Train model to maximize likelihood $\mathcal{P}_{\theta}(Y | [P_{S(t)}; X])$ with $\theta$ fixed
    \EndFor
    \State Return domain-specific prompts $P_{S1}, P_{S2}, \ldots, P_{S\tau}$
\EndProcedure

\Procedure{TemporalPromptLearning}{}
    \State Initialize the temporal prompt generator $g_\omega$
    \For{each domain $D_t$ in $\{D_t | 2 \leq t \leq \tau+1\}$}
        \State Provide prompts $P_{S1}, P_{S2}, \ldots, P_{S(t-1)}$ to temporal prompt generator $g_\omega$
        \State Generate temporal prompt   $P_{T(t)}$
        \State Prepend input $X$ from domain $t$ with $P_G$ and $P_{T(t)}$
        \State Process input $[P_{T(t)}; P_G; X]$ using frozen backbone $f_\theta$
        \State Train model to maximize likelihood $\mathcal{P}_{\theta}(Y | [P_{T(t)}; P_G; X])$ with $\theta$ fixed
    \EndFor
    
  
\EndProcedure

\end{algorithmic}
\end{algorithm*}


==> sections/conclusion.tex <==
\section{CONCLUSION}

%The efficacy of machine learning often depends on data distribution assumptions, which can be challenged by distribution and concept drifts. This paper studied the situation when data distribution evolves temporally. Such temporal drifts emphasize the need for temporal domain generalization (DG). Our work introduces a parameter and time-efficient prompting-based temporal DG method, bridging gaps in applicability across tasks like time series forecasting . This represents a significant stride toward anticipating and adapting models to future domains using previous domains information.

The efficacy of machine learning often depends on the assumptions that training and testing data are distributed independently and identically, an assumption that can be challenged by distribution shifts and concept drifts. This paper studied the scenarios where data distribution evolves over time. Such temporal drifts emphasize the need for temporal domain generalization (DG). In this paper, we propose a parameter and time-efficient prompting-based Temporal DG method that adeptly adapts pre-trained models to unforeseen future domains across various tasks, encompassing classification, regression, and time series forecasting. This represents a significant stride toward anticipating and adapting models to future domains using previous domains information.


==> sections/intro.tex <==
\section{Introduction}
Machine learning has achieved great success in many applications in recent years, and most machine learning algorithms rely on the assumption that the training (i.e. source) and test (i.e. target) data are independently and identically distributed (i.i.d.). However, in reality, distribution shift and concept drift are often observed, and these non-i.i.d problems are more challenging to tackle. In domain adaptation (DA), extensive research has been conducted on adapting models to the target domain by modelling the domain relations between the source and the target~\cite{courty2016optimal,gong2012geodesic,hoffman2014continuous,jimenez2019cdot,lao2020continuous,wang2020continuously,yang2016multivariate}. However, such models assume that target domain data is available, which may not always hold in real-world settings. Domain generalization (DG) methods tackle the scenario where models are directly generalized to the target domain without the presence of the target data (labelled or unlabelled)~\cite{yue2019domain,prakash2019structured,shankar2018generalizing,volpi2018generalizing,hu2021domain,triantafillou2021learning,kim2021self,wang2020meta}.


DG traditionally focuses on generalization among categorical-indexed domains with categorical task~\cite{wang2021generalizing,chen2022mix}. In contrast, \emph{temporal DG} addresses the continuously time-evolving distribution shift (namely concept drift) problem~\cite{bai2023temporal, nasery2021training}.
For example, suppose we would like to predict house prices given information about the property's physical characteristics, such as square footage, number of bedrooms, number of bathrooms, and location. Since house prices are influenced by macroeconomic conditions and demographic trends that change over time, a regression model trained on data collected from the past few years could have poor predictive power next year~\cite{yin2022spatial}. However, suppose the macroeconomic and demographic factors change gradually over time. In that case, we can extrapolate their influence into the short-term future, and adapt the regression model to make more accurate predictions. Such cases are where temporal domain generalization can be applied. For example, suppose we know that the population in a particular country has been steadily aging over the past several years, which reduces the overall demand for many-bedroom houses. A temporal DG algorithm can anticipate that the demand will continue to fall for many-bedroom houses and adapt the price predictions for these houses accordingly: given the same features, a many-bedroom house next year will be priced some amount less than this year. Note that in the temporal DG setting, we do not get to see the ``test domain", i.e., next year's house prices, during training. Therefore, temporal DG methods that model the continuously time-evolving data dynamics and generalize well to the future are needed.

Most standard DG methods cannot be directly applied to temporal DG. Different from standard DG problems, which aim to discover general representations among different domains and learn domain-invariant features, capturing the temporal dynamics of domain data changing over time is crucial for temporal DG. Learning domain-invariant features, namely time-invariant representations in temporal DG case, no longer work. Only a few methods studied temporal DG problem~\cite{nasery2021training, bai2023temporal}, which are inefficient and complex to be applied to large datasets and large models. Moreover, all the prior works only showed their effectiveness on classification and/or regression tasks, while missing demonstrations on other applications, such as time series forecasting. Therefore, a more efficient temporal DG framework enabling more diverse tasks is valuable.



Prompting is well-known for efficiently adapting a trained network to different tasks without retraining~\cite{lester2021, vu2021spot, gu2021ppt, li2021prefix, asai2022attempt,wang2023multitask}. Most prior works~\cite{jia2022prompt,zhang2021domain,li2022learning,dunlap2022using,pmlr-v202-shu23a} adopting prompting for DG are applicable to only CLIP~\cite{radford2021learning} and cannot be applied to other architectures or tasks. PADA~\cite{ben2022pada} is a recent work proposed for DG. It first generates example-specific prompts, and then the generated prompts are applied to T5 for classification tasks. However, PADA is applicable only to classification tasks, and it can only generate word tokens as prompts.

Moreover, none of these prior works can generate time-sensitive prompts that capture temporal dynamics. In this paper, we proposed a parameter-efficient and time-efficient prompting-based temporal DG method. To capture temporal dynamics, domain-specific prompts are first generated on each domain. Then, our method learns time-sensitive prompts by modelling the temporal changes from domain-specific prompts and forecasts future prompts for unseen future domains. Our method also learns global prompts shared across all domains to learn generic representations. The prompts are generated in vector space and can be applied to a wide range of network architectures.


To sum up, our contributions are:
(1) We propose the first prompting-based temporal DG method for addressing data distribution shifts over time. (2) Our method is parameter-efficient and time-efficient. In contrast to the state-of-the-art approach~\citep{bai2023temporal}, which generates a full network for each domain, including the target domain, only a few parameters shared across all domains are allocated for prompt generation, and no additional parameters are needed for the target domain. (3) Our method is general and can be applied to many applications, including classification, regression, and time series forecasting.
  

==> sections/preliminary_icml.tex <==
\section{Preliminaries: prompt-tuning}
Large language models (LLMs) trained on massively large data sets are known to be very effective in understanding given content and generating new content. However, adapting trained LLMs to downstream tasks is computationally expensive and time consuming given the large amount of parameters. Prompt tuning is a technique adapting LLMs to downstream tasks efficiently. More specifically, prompt tuning contains two main components: prompts and a frozen backbone transformer network. The prompts are prepended to the inputs, guiding the frozen transformer in adapting to different downstream tasks. There are different types of prompts: hard prompts refer to manually crafted and non-learnable text such as class name~\cite{jia2022prompt} prepended to the inputs, soft prompts are learnable vectors prepended to the inputs~\cite{lester2021, vu2021spot, gu2021ppt}, and prefix prompts are learnable vectors injected to more layers in the frozen backbone~\cite{li2021prefix}. Note that the backbone transformer is fixed in all settings and only prompts are possible learnable parameters.

